Random Hyperbolic Graphs: Degree Sequence and Clustering

In the last decades, the study of models for large real-world networks has been a very popular and active area of research. A reasonable model should not only replicate all the structural properties that are observed in real world networks (for example, heavy tailed degree distributions, high clustering and small diameter), but it should also be amenable to mathematical analysis. There are plenty of models that succeed in the first task but are hard to analyze rigorously. On the other hand, a multitude of proposed models, like classical random graphs, can be studied mathematically, but fail in creating certain aspects that are observed in real-world networks. Recently, Papadopoulos, Krioukov, Boguna and Vahdat [INFOCOM'10] introduced a random geometric graph model that is based on hyperbolic geometry. The authors argued empirically and by some preliminary mathematical analysis that the resulting graphs have many of the desired properties. Moreover, by computing explicitly a maximum likelihood fit of the Internet graph, they demonstrated impressively that this model is adequate for reproducing the structure of real graphs with high accuracy. In this work we initiate the rigorous study of random hyperbolic graphs. We compute exact asymptotic expressions for the expected number of vertices of degree k for all k up to the maximum degree and provide small probabilities for large deviations. We also prove a constant lower bound for the clustering coefficient. In particular, our findings confirm rigorously that the degree sequence follows a power-law distribution with controllable exponent and that the clustering is nonvanishing.

==> main_result.tex <==
\subsection{The Average \& Maximum Degree}
In the subsequent proofs for Theorem~\ref{thm:average_degree} and Theorem~\ref{thm:max_degree}, we present two simple applications of Lemma~\ref{lem:intersection_area}. In particular, we show how it can be used to determine the average degree and the maximum degree in $G_{\alpha, C}(n)$.

\begin{proof}[Proof of Theorem~\ref{thm:average_degree}]
The average degree of a fixed vertex at radius $r$ is by definition 
\begin{equation}
\label{eq:avgkr}
\overline{k}(r)= (n-1) \mu(B_r(R)\cap B_0(R))\stackrel{\text{(Lem.\ \ref{lem:intersection_area})}}{=}(n-1) \left( \frac{2\alpha e^{-r/2}}{\pi(\alpha-1/2)} \Bigl(1\pm O\bigl(e^{-(\alpha-1/2)r}+e^{-r}\bigr)\Bigr) \right).
\end{equation}
The total average degree can be obtained by integrating $\overline{k}(r)p(r)$ over all $0 \le r\le R$. With the facts $2\sinh(x) = e^x(1 - \Theta(e^{-2x}))$ and $2\cosh(x) = e^x(1 + \Theta(e^{-2x}))$, valid for any $x \ge 0$, it follows that
\begin{equation}
\label{eq:prestimate}
	p(r)
	= \frac{ \alpha\sinh(\alpha r)}{\cosh(\alpha R)-1}
	= \alpha e^{\alpha(r-R)} \cdot (1 \pm O(e^{-2\alpha r} + e^{-\alpha R}))
\end{equation}
Note that since $\alpha > 1/2$ and $0 \le r \le R$, the error terms $e^{-2\alpha r} + e^{-\alpha R}$ in~\eqref{eq:prestimate} are dominated by the error terms $e^{-(\alpha-1/2)r}+e^{-r}$ in~\eqref{eq:avgkr}. Hence, by abbreviating $c_\alpha = \frac{2\alpha^2}{\pi(\alpha - 1/2)}$ we obtain
\begin{align*}
\overline{k}
&= \int_0^Rp(r)\overline{k}(r)dr
= (1+o(1)) c_\alpha n \int_0^R  e^{\alpha(r-R)}\cdot e^{-r/2}\left(1 \pm O\left(e^{-(\alpha-1/2)r} + e^{-r}\right)\right) dr.
\end{align*}
The last integral is elementary. In particular, recalling that $R = 2\log n + C$, we obtain that
\[
	\int_0^R  e^{\alpha(r-R)}\cdot e^{-r/2} dr
	= 
	\frac{e^{-\alpha R}}{\alpha - 1/2} \left[e^{(\alpha - 1/2)r}\right]_{r=0}^R
	=
	(1+o(1))\frac{e^{-R/2}}{\alpha - 1/2}
	= (1+o(1))\frac{n^{-1}e^{-C/2}}{\alpha - 1/2}.
\]
The integrals over the error terms are of order
$$O\left(n\int_0^Re^{\alpha(r-R)}e^{-r/2}e^{-(\alpha -1/2)r}dr \right)=O\left(n e^{-\alpha R}\int_0^Rdr \right)=o(1) $$
and
$$O\left(n e^{-\alpha R}\int_0^R e^{r(\alpha -3/2)}dr\right)=O\left(ne^{-\alpha R}e^{R(\alpha -3/2)}\right)=o(1).$$
%Soda only
%The integrals containing the error terms, as they also contain only elementary functions, can be easily shown to be of lower order compared to the expression above.
Finally,
\[
	\overline{k} = (1+o(1)) \frac{c_\alpha \, e^{-C/2}}{\alpha-1/2} = (1+o(1))\frac{2\alpha^2\, e^{-C/2}}{\pi(\alpha - 1/2)^2},
\]
and the theorem follows.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:max_degree}]
Let $X_{\le r}$ denote the number of vertices with radius at most $r$, and define $X_{\geq r}$ similarly. Set $r_0:=(2-1/\alpha)\log n$. We will consider vertices with radius $r\in [r_0-\phi(n), r_0+\phi(n)]$ where $\phi(n)=o(\log \log n)$  tends to infinity as $n\rightarrow \infty$. Note that for sufficiently large $n$
\begin{equation}
\label{eq:max_degree_no_vertices_inside}
\mathbb{E}[X_{\le r_0-\phi(n)}]= n\cdot \mu\left(B_0\left(r_0-\phi(n)\right)\right)\stackrel{(\text{Lem.\ \ref{lem:intersection_area}})}{\le} 2 e^{-\alpha (\phi(n)+C)}=o(1).
\end{equation}
It follows that with high probability there are no vertices with radius at most $r_0-\phi(n)$. Moreover, by applying~\eqref{eq:ball-area}
\begin{equation}
\label{eq:massr0bounds}
\frac{e^{\alpha (\phi(n)-C)}}{2n}\le \mu\left(B_0(r_0+\phi(n))\right)\le \frac{2e^{\alpha (\phi(n)-C)}}{n}.
\end{equation}
Since the number of vertices with radius $\le r_0 + \phi(n)$ is binomially distributed, we infer that
\begin{equation}
\label{eq:max_degree_vertices_inside}
\Pr[X_{\le r_0+\phi(n)}=0]\le \left(1- \mu(B_0(r_0+\phi(n))) \right)^n\le e^{-{e^{\alpha (\phi(n)-C)}}/{2}}=o(1).
\end{equation}
That is, with high probability there is a vertex with radius at most $r_0+\phi(n)$. On the other hand, we will argue that the number of such vertices is very small. To see this, note that~\eqref{eq:massr0bounds} implies that
$$\mathbb{E}[X_{\le r_0+\phi(n)}]\le 2e^{\alpha( \phi(n)-C)},$$
and by applying Markov's inequality we infer, since $\phi(n) = o(\log\log n)$, that
$$\Pr[X_{\le r_0+\phi(n)}>\log n] \le \frac{2e^{\alpha(\phi(n)-C)}}{\log n}=o(1).$$
In other words, the number of vertices with radius larger than $r_0 + \phi(n)$ is at least $n - \log n$ with high probability.

Note that the degree of a vertex at radius $r$ is distributed like $\textrm{Bin}\bigl(n-1, \mu(B_0(R)\cap B_r(R))\bigr)$. As there are with high probability no vertices of radius smaller than $r_0-\phi(n)$, by Lemma~\ref{lem:monotone} the degree distribution of every vertex is with high probability dominated by $\textrm{Bin}(n, p_{r_0}^-)$, where by Lemma~\ref{lem:intersection_area}
$$p_{r_0}^- :=\mu(B_0(R)\cap B_{r_0-\phi(n)}(R))=(1+o(1))\frac{2\alpha}{\pi(\alpha-1/2)}e^{-\frac{r_0-\phi(n)}{2}}.$$
In this case the expected degree of a fixed vertex is at most $np_{r_0}^-\le (1+o(1))\frac{2\alpha}{\pi(\alpha -1/2)}n^{\frac{1}{2\alpha}}e^{\frac{\phi(n)}{2}}$ and by a Chernoff bound and a union bound there is with high probability no vertex of degree larger than $(1+o(1))\frac{4e\alpha}{\pi(\alpha-1/2)}n^{\frac{1}{2\alpha}}e^{\frac{\phi(n)}{2}}$.

The lower bound can be established by the fact (shown in \eqref{eq:max_degree_vertices_inside}) that there is with high probability a vertex of radius at most $r_0+\phi(n)$. There are with high probability at most $\log n$ such vertices which means that we can fix one and have that by Lemma~\ref{lem:monotone} its degree distribution dominates $\textrm{Bin}(n-\log n, p_{r_0}^+)$ where by Lemma~\ref{lem:intersection_area} 
$$p_{r_0}^+:=\mu(B_0(R)\cap B_{r_0+\phi(n)}(R)\setminus B_0(r_0+\phi(n)))=(1+o(1))\frac{2\alpha}{\pi(\alpha-1/2)}e^{-\frac{r_0+\phi(n)}{2}}.$$
Note that the expectation of $\textrm{Bin}(n-\log n, p_0^+)$ is $(1+o(1))np^+_0=(1+o(1))\frac{2\alpha}{\pi(\alpha -1/2)}n^{\frac{1}{2\alpha}}e^{-\frac{\phi(n)}{2}}$ and is therefore by a Chernoff bound with high probability not smaller than $\frac{\alpha}{\pi(\alpha-1/2)}n^{\frac{1}{2\alpha}}e^{-\frac{\phi(n)}{2}}$.
\end{proof}


\subsection{Vertices of Small Degree }

In this section we prove the first part of Theorem~\ref{thm:degree_seq}. Before we give all technical details, let us describe briefly the main proof idea. Given the estimates in the previous sections, in particular Lemma~\ref{lem:intersection_area}, it is conceptually not very difficult to compute the expected number of vertices of degree $k$ in $G_{\alpha, C}(n)$. Nevertheless, it is not clear how to show the claimed strong concentration bound. To this end, we will apply an Azuma-Hoeffding-type large deviation inequality, see Lemma~\ref{lem:concentration} below.

In a typical setting, such concentration inequalities require some kind of \emph{Lipschitz condition} that is satisfied by the function under consideration. In our specific setting, the function counts number of vertices of degree $k$, and it is required to provide a bound for the maximum effect that any vertex has on it. However, the only a priori bound that can be guaranteed is that the number of vertices of degree $k$ can change by at most $n$, as a vertex may connect or not connect to any other vertex. To make the situation worse, this bound is even tight, since a vertex can be placed at the center of disc, i.e., if it has radial coordinate equal to 0.

We will overcome this obstacle as follows. Instead of counting the total number of vertices of degree $k$, we will consider only vertices that lie far away from the center of the disc, i.e., which have radial coordinate larger that $\beta R$, for some appropriate $\beta >0$. Moreover, we will consider only vertices such that all their neighbors have a large radial coordinate as well. This restriction will allow us to bound the maximum effect on the target function, as with high probability all these vertices do not have too large degree.

More formally, we proceed as follows. We partition the vertex set of $G_{\alpha, C}(n)$ into two sets. The \emph{inner set} $I = I(\beta)$ contains all vertices of radius at most $\beta R$ while the \emph{outer set} $O = O(\beta)$ contains all vertices of radius larger than $\beta R$. Moreover, let $e(I,O)$ count the number of edges with one endpoint in $I$ and the other in $O$. The next two lemmas show that $e(I,O)$ and $|I|$ are small. This indicates that most of the vertices of degree $k$, for not too large $k$, will lie in $O$. Let $D_k$ denote the number of vertices in $O$ which have degree $k$ in $O$, i.e., set 
$$D_k(\beta) = \left|\big\{v\in O(\beta) ~\big|~ |N(v) \cap O(\beta)| = k \big\}\right|.$$
In Lemma~\ref{lem:degree_sequence} we derive the expectation of $D_k$ and show then in Lemma~\ref{lem:lipschitz} that unless something very unlikely happens (namely that there is a vertex of large degree in $O$) the effect of every point in $O$ on $D_k$ is small. This allows us to apply a Azuma-like inequality (Lemma~\ref{lem:concentration}) to show that $D_k$ is tightly concentrated around its expectation. 

\begin{figure}
\begin{center}
  \begin{tikzpicture}[dot/.style={draw, circle,inner sep=1pt,fill},scale=0.4]
    \def\rad{3cm};
    \filldraw[fill=gray!20] (0,0) circle (2cm);
    \node[dot] (c) at (0,0) {};
    \draw (c) circle (\rad);
    \draw[latex-latex] (c) -- node[pos=0.55,right] {\(R\)} (120:\rad);
    \draw[latex-latex] (c) -- node[below] {\(\beta R\)} (20:2cm);
    \node (i) at (0,-1) {\(I\)};
    \node (o) at (0,-2.5) {\(O\)};
  \end{tikzpicture}
\end{center}
\caption{\small The partitioning of the disk into two sets $I$ and $O$.\label{fig:io}}
\end{figure}


\begin{lemma}
\label{lem:few_vertices_I}
In $G_{\alpha, C}(n)$, with  probability at least $1 - e^{-n^{\Omega(1)}}$
$$|I(\beta)| \le \max\{n^{1/2}, 4en^{1-2\alpha (1-\beta)}e^{-\alpha C(1-\beta)}\}.$$
\end{lemma}
\begin{proof}
The number of vertices in $I$ is distributed like $\textrm{Bin}(n, \mu\bigl(B_0(\beta R)\bigr))$. Therefore the expected number of vertices in $I$ is (by  Lemma~\ref{lem:intersection_area}) bounded by 
$$\mathbb{E}[|I(\beta)|]\le  n \mu\bigl(B_0(\beta R)\bigr) = (1+o(1))ne^{-\alpha(R-\beta R)}\le 2n^{1-2\alpha (1-\beta)}e^{-\alpha C(1-\beta)}$$
and it follows by the Chernoff bound that for $t=\max\{n^{1/2}, 4en^{1-2\alpha (1-\beta)}e^{-\alpha C(1-\beta)}\}$
$$\Pr[|I(\beta)| >t]\le 2^{-t}=e^{-n^{\Omega(1)}}.$$
\end{proof}

\begin{lemma}
\label{lem:few_edges_IO}
Let $\varepsilon>0$ and $0<\beta<1$. Then it holds with high probability that
$$e(I(\beta),O(\beta))= O\left( n^{1-(2\alpha-1)(1-\beta)}\log n\right).$$
\end{lemma}

\begin{proof}
Let $r_0:=\left(1-\frac{1}{2\alpha}\right)\log n+C$ and note that by Lemma~\ref{lem:intersection_area} the expected number of vertices of radius at most $r_0$ is at most
$$n\mu(B_0(r_0))=(1+o(1))ne^{-\alpha(R-r_0)}=ne^{-(\alpha+1/2)\log n} =o(1).$$
We therefore have with high probability no vertex of radius at most $r_0$. For all $r_0\le r\le \beta R$ we get by Lemma~\ref{lem:intersection_area} that the expected degree in $O$ of a vertex at radius $r$ is at most
\begin{equation}
\label{eq:expected_o_deg_of_r}
n\mu(B_r(R)\cap B_0(R)\setminus B_0(\beta R)) = O\left(ne^{-r/2}\right).
\end{equation}
We now integrate over \eqref{eq:expected_o_deg_of_r} in $I$ to bound the expected number of edges between $I$ and $O$. Recall that there are with high probability no vertices of radius at most $r_0$ and it therefore suffices to integrate from $r_0$ to $\beta R$ 
\begin{align*}O\left(n^2\int_{r_0}^{\beta R} e^{-r/2}p(r)dr \right) &= O\left(n^{2}e^{-\alpha R}\int_0^{\beta R}e^{(\alpha-1/2)r}dr \right)=O\left(n^{2-2\alpha+2\beta(\alpha -1/2)} \right)\\
&=O\left( n^{1-(2\alpha-1)(1-\beta)}\right).
\end{align*}
The lemma follows by Markov's inequality. 

\end{proof}

%%%%%%%%%%%%%  Old Proof using the stripes for exponential concentration (which we can't get!)
%\begin{proof}
%We partition the vertices in $I$ into disjoint sets $S_1, \dots, S_t$. Let $r_0:=\frac{2\alpha-1-\varepsilon}{\alpha}\log n$ and for all $1\le i \le t$  define $r_i:=\frac{2\alpha-1+\varepsilon}{\alpha}\log n+\frac{\log i}{\alpha}$.
%For $1\le i\le t$ let $S_i$ contain all vertices which are in $B_0(r_i)\setminus B_0(r_{i-1})$ and let $S_0$ contains all vertices in $B_0(r_0)$. 
%Note that by Lemma~\ref{lem:intersection_area} for all $1\le i \le t$ we have that 
%$$\mu(S_i)=\mu(B_0(r_i)) -\mu(B_0(r_{i-1}))=(1+o(1))e^{-\alpha R}(e^{\alpha r_i}-e^{\alpha r_{i-1}})=(1+o(1))n^{-1+\varepsilon}$$
%and we have that 
%$$ \mu(S_0)=\mu(B_0(r_0))=(1+o(1))e^{-\alpha(R-r_0)}=(1+o(1))n^{-1-\varepsilon}\enspace.$$
%Therefore, the number of vertices of $G_{\alpha, C}(n)$ is $S_i$ satisfies
%$$\mathbb{E}[|V \cap S_i|]=(1+o(1))n^{\varepsilon} \enspace,$$
%i.e., we expect roughly $n^\varepsilon$ vertices in $S_i$.
%It remains to specify $t$. Note that $t$ satisfies
%$ r_{t} = \beta R$, which can be rearranged to give
%$$t=n^{-2\alpha (1-\beta)+(1-\varepsilon)}\cdot e^{\beta C} \enspace.$$
%The quantity $|V \cap S_i|$ is binomially distributed. By appling a Chernoff bound, and subsequently a union bound over all vertices we infer that with probability at least $1-2^{-2en^{\varepsilon}+\log_2n}$ it holds that  $|V \cap S_i| \le 2en^{\varepsilon}$ for all $1\le i\le t$.

%Next we consider the number of neighbors of each vertex in $S_i$ in $O(\beta)$.
%By applying Lemma~\ref{lem:intersection_area} and Lemma~\ref{lem:monotone} we infer that there is a constant $c'>0$ such that the expected degree in $O(\beta)$ of a vertex in $S_i$ (for $2\le i\le t$ ) is at most
 %\begin{equation}
 %\label{eq:mass_s1}
 %n \cdot \mu(B_{r_{i-1}}(R)\cap B_0(R)\setminus B_0(\beta R))\le c'ne^{-\frac{r_{i-1}}{2}} \le c\, {(i-1)^{-{1}/{2\alpha}}}\, n^{(1-\varepsilon)/{2\alpha}}
 %\end{equation}
%and for a vertex in $S_1$ it is at most
 %  \begin{equation}
 %\label{eq:mass_si}
 % n \cdot \mu(B_{r_{0}}(R)\cap B_0(R)\setminus B_0(\beta R))\le c'ne^{-\frac{r_{0}}{2}}=cn^{\frac{1+\varepsilon}{2\alpha}}\enspace.
  %\end{equation}
%By the same argument as before it holds with probability exponentially close to $1$ that no $S_i$ contains a vertex which is more than a factor of $2e$ larger than the right hand side of \eqref{eq:mass_si} (respectively  \eqref{eq:mass_s1}). We conclude that there is a $\varepsilon':= \varepsilon'(\varepsilon)$  such that the number of edges between $I$ and $O$ is with probability at least $1-e^{n^{\varepsilon'}}$ at most
%\marginpar{\tiny Kosta: benutzt du hier dass $S_0$ leer ist?}
%\begin{align*}
%\sum_{i=1}^{t} e(S_i, O)&\le 4cn^{\varepsilon +\frac{1-\varepsilon}{2\alpha}} \left(n^{\frac{2\varepsilon}{2\alpha}}+ \sum_{i=2}^t\frac{1}{(i-1)^{\frac{1}{2\alpha}}}\right)\le 4cn^{\varepsilon +\frac{1-\varepsilon}{2\alpha}} \left(n^{\frac{2\varepsilon}{2\alpha}}+ \int_{i=0}^{t-2}\frac{1}{(i-1)^{\frac{1}{2\alpha}}}\right)\\
%&=4cn^{\varepsilon +\frac{1-\varepsilon}{2\alpha}} \left(n^{\frac{2\varepsilon}{2\alpha}}+ \left[\frac{i^{1-\frac{1}{2\alpha}}}{1-\frac{1}{2\alpha}} \right]^{t-2}_0\right) =4cn^{\varepsilon +\frac{1-\varepsilon}{2\alpha}} \left(n^{\frac{2\varepsilon}{2\alpha}}+ \frac{2\alpha}{2\alpha -1}\left(t^{1-\frac{1}{2\alpha}}-1 \right)\right)\\
%&\le 4cn^{\varepsilon+\frac{1+\varepsilon}{2\alpha}}+\frac{8\alpha c}{2\alpha -1} n^{1-(2\alpha -1)(1-\beta)}e^{\beta C \frac{2a-1}{2\alpha}}\enspace.
%\end{align*}
%\marginpar{\tiny Kosta: argh, hier integrierst du ueber undefinierte Stellen!}
%\end{proof}

In the next lemma we derive the expected degree sequence of the subgraph spanned by $O$.

\begin{lemma}
\label{lem:degree_sequence}
Let $\alpha > 1/2, C\in \mathbb{R}$, and $\max\left\{3/5, 1/(2\alpha)\right\} < \beta <1$. Set $\delta:=\min\{2(2\beta-1), 1/2\}$. Then, for all $0 \le k = o(n^\delta)$ we have that
$$\mathbb{E}[D_k(\beta)]=  \bigl(1+o(1)\bigr)\frac{2n\alpha e^{-\alpha C}}{k!} \Bigl(\frac{2\alpha}{\pi(\alpha-1/2)}\Bigr)^{2\alpha}\left( \Gamma(k-2\alpha)-\int_{0}^{\xi} t^{k-2\alpha-1}e^{-t}dt  \right),$$
where
$
	\xi = \frac{2\alpha}{\pi(\alpha - 1/2)} e^{-C/2}.
$
\end{lemma}

\begin{proof}
  Let \(p = (r, \theta)\) be an arbitrary fixed vertex with \(r > \beta R\).
  Denote with \(\bar{q}_r\) the probability that a random vertex \(p' = (r',
  \theta')\) has radius at least \(\beta R\) and distance at most \(R\) from
  \(p\). We have that
  \begin{equation*}
    \bar q_r = \mu\bigl((B_r(R) \cap B_0(R))\setminus B_{0}(\beta R)\bigr) .
  \end{equation*}
  The probability that \(p\) has \(k\) neighbors with radius larger than $\beta R$ then corresponds to
  the probability that a binomial random variable \(\Bin(n-1,\bar{q}_r)\) has
  value \(k\). Therefore the expected value of \(D_k\) can be computed by
  \begin{equation}
    \label{eq:deg_seq_exp}
    \mathbb{E}[D_k] =  n\int_{\beta R}^R
    \binom{n-1}{k}\bar{q}_r^k(1-\bar{q}_r)^{n-1-k} p(r) dr .
  \end{equation}
  By Lemma \ref{lem:intersection_area}, Equation~\eqref{eq:massComp}, and the observation that $\Theta(e^{-2\alpha \beta R})=O(e^{-r})$ it follows that
  \begin{equation*}
    \bar q_r = \frac{2\alpha e^{-r/2}}{\pi(\alpha-1/2)} \Bigl(
    1-e^{-(\alpha-1/2)(1-\beta)R}\Bigr)\Bigl(1 \pm O\bigl(e^{-r}+e^{-r-(\alpha-3/2)(1-\beta)R}\bigr)
    \Bigr).
  \end{equation*}
  Recall that \(R = 2\log n+C\) and
  therefore \(e^{-r} \leq e^{-\beta R} = o(1/n)\).  
  To approximate the integral in Equation~\eqref{eq:deg_seq_exp} we separate
  the main and error terms as follows. Write
  \begin{equation*}
    q_r = \frac{2\alpha e^{-r/2}}{\pi(\alpha-1/2)} \Bigl(
    1-e^{-(\alpha-1/2)(1-\beta)R}\Bigr) \quad\text{and}\quad
    f_r = O\bigl(e^{-r-(\alpha-3/2)(1-\beta)R}\bigr)+o(1/n) .
  \end{equation*}
	Note that $\bar q_r = q_r (1 \pm f_r) $.
	Before we proceed with the estimation of the expression in~\eqref{eq:deg_seq_exp} let us prove some auxiliary facts. For all~\(r > \beta R\) and all~\(\alpha > 1/2\) we claim to have the following
  properties for \(q_r\), \(f_r\) and \(k\):
\begin{equation}
\label{eq:aux_prop}
  \textrm{i)}~q_r f_r = o(1/n),
  \qquad\textrm{ii)}~(q_r)^2 = o(1/n),
  \qquad\textrm{ and \qquad iii)}~f_r k = o(1).
\end{equation}
  Property i) is established by observing that whenever $\beta > 3/5$
  \begin{equation*}
    q_rf_r = O\bigl(e^{-(\alpha-3/2)(1-\beta)R-r/2-r}\bigr)
    \stackrel{(r \ge \beta R)}{=} O\bigl(e^{-(\alpha-3/2)(1-\beta)R-{3\beta R}/{2}}\bigr)
    = O\bigl(n^{3 - 6\beta - 2\alpha + 2\alpha\beta}\bigr) = o(1/n).
  \end{equation*}
  The second claimed property is true because \((q_r)^2 = O(e^{-\beta R}) = O(n^{-2\beta})=O(n^{-6/5})\),
  while the third is satisfied by our choice of \(k=o(n^{2(2\beta-1)})\). We claim that these facts imply
  \begin{equation}\label{eq:degseq-approx-integral}
    n\int_{\beta R}^R
    \binom{n-1}{k}(\bar{q}_r)^k(1-\bar{q}_r)^{n-1-k} p(r) dr =
    \bigl(1+o(1)\bigr)\frac{n}{k!}
    \int_{\beta R}^R
    (n q_r)^ke^{-n q_r} p(r) dr.
  \end{equation}
  Consider first the binomial coefficient. Since $k \ll \sqrt{n}$ we have
  \begin{equation*}
    \binom{n-1}{k} = \frac{(n-1)^k}{k!} \, \prod_{i=0}^{k-1}\left(1 - \frac{i}{n-1}\right) = \bigl(1+o(1)\bigr)\frac{n^{k}}{k!}.
  \end{equation*}
  Next we consider the term \((\bar q_r)^k\). By using the third property in~\eqref{eq:aux_prop} we obtain that
  \begin{equation*}
    (\bar q_r)^k = (q_r(1+f_r))^k = (q_r)^k\bigl(1+\Theta(f_r k)\bigr) =
    (1+o(1))(q_r)^k.
  \end{equation*}
  Finally, we have that
  \begin{equation*}
    \begin{split}
      (1-\bar q_r)^{n-1-k} &~~=~~ (1-q_r)^{n-1-k}\bigl(1 +
      q_rf_r/(1-q_r)\bigr)^{n-1-k} \\
      &~~=~~ e^{(n-1-k)\log(1-q_r)}(1+\Theta(n q_rf_r))\\
      &\stackrel{\eqref{eq:aux_prop}, i)}{=} e^{-n q_r+O((n-1-k)q_r^2)+(k+1)q_r}\bigl(1+o(1)\bigr)\\
      &\stackrel{\eqref{eq:aux_prop}, ii)}{=} e^{-n q_r}(1+o(1)).
    \end{split}
  \end{equation*}
  This completes the proof of~\eqref{eq:degseq-approx-integral}. We now estimate the integral on the right hand side of
  Equation~\eqref{eq:degseq-approx-integral}. To do so we first perform a
  variable transformation \(t = nq_r\). Then, the density \(p(r)\)
  can be expressed as
  \begin{equation*}
    \begin{split}
      p(r) &= \frac{\alpha\sinh(\alpha r)}{\cosh(\alpha R)-1} =
      \frac{\alpha}{2(\cosh(\alpha R)-1)}\bigl(e^{\alpha r}- e^{-\alpha
        r}\bigr)\\
      &= \frac{\alpha}{2(\cosh(\alpha R)-1)}
      \left((nq_r)^{-2\alpha}n^{2\alpha}
      \left(\frac{2\alpha \left(
    1-e^{-(\alpha-1/2)(1-\beta)R}\right) }{\pi(\alpha-1/2)}\right)^{2\alpha}-o(1)\right)\\
  \end{split}
  \end{equation*}
Since \(1/(\cosh(\alpha R)-1) =
  2n^{-2\alpha}e^{-\alpha C}\bigl(1+o(1/n)\bigr)\), the above calculation yields that
\[
	p(r) = \alpha e^{-\alpha C} \Bigl(\frac{2\alpha}{\pi(\alpha-1/2)}\Bigr)^{2\alpha}
      (nq_r)^{-2\alpha}\bigl(1+o(1)\bigr).
\]
Further we have that
  \begin{equation*}
    dt = n\frac{2\alpha\left(
    1-e^{-(\alpha-1/2)(1-\beta)R}\right)}{\pi(\alpha-1/2)}(-1/2)e^{-r/2}dr =
    -\frac{1}{2}t dr\quad\Rightarrow\quad dr = -2t^{-1}dt,
  \end{equation*}
  and for the upper and lower bounds that
  \begin{equation*}
    \begin{split}
      r_0 = \beta R \quad&\longrightarrow\quad t_0 = n
      \frac{2\alpha\left(
    1-e^{-(\alpha-1/2)(1-\beta)R}\right)}{\pi(\alpha-1/2)} e^{-\beta R/2} =
      \frac{2\alpha\left(
    1-e^{-(\alpha-1/2)(1-\beta)R}\right)}{\pi(\alpha-1/2)} e^{-\frac{\beta C}{2}}n^{1-\beta}\\
      r_1 = R \quad&\longrightarrow\quad t_1 = n
      \frac{2\alpha\left(
    1-e^{-(\alpha-1/2)(1-\beta)R}\right)}{\pi(\alpha-1/2)} e^{-R/2} =
      \frac{2\alpha\left(1-e^{-(\alpha-1/2)(1-\beta)R}\right)}{\pi(\alpha-1/2)}e^{-C/2}.
    \end{split}
  \end{equation*}
  Putting everything together we have that the right hand side of~(\ref{eq:degseq-approx-integral}) can be approximated by
  \begin{multline*}
    \bigl(1+o(1)\bigr)
    \frac{2n\alpha e^{-\alpha C}}{k!}
    \Bigl(\frac{2\alpha}{\pi(\alpha-1/2)}\Bigr)^{2\alpha}
    \int_{t_1}^{\infty}
    t^{k-2\alpha-1}e^{-t}dt \\
%  =    \bigl(1+o(1)\bigr)
%    \frac{2n\alpha e^{-\alpha C}}{k!}
%    \Bigl(\frac{2\alpha}{\pi(\alpha-1/2)}\Bigr)^{2\alpha}
%    \left(\int_{0}^{\infty}
%    t^{k-2\alpha-1}e^{-t}dt -\int_{0}^{t_1} t^{k-2\alpha-1}e^{-t}dt  \right)\\
  =  \bigl(1+o(1)\bigr)
    \frac{2n\alpha e^{-\alpha C}}{k!}
    \Bigl(\frac{2\alpha}{\pi(\alpha-1/2)}\Bigr)^{2\alpha}
    \left( \Gamma(k-2\alpha)-\int_{0}^{t_1} t^{k-2\alpha-1}e^{-t}dt  \right).
  \end{multline*}
The proof is completed with the observation $t_1 = (1 - o(1))\xi$.
\end{proof}

%Note that by Sterling's approximation for $k=\omega(1)$
%$$k!=\sqrt{2\pi k}\left(\frac{k}{e} \right)^k(1+o(1)) $$
%and
%$$\Gamma(k-2\alpha) = \sqrt{2\pi (k)}\left(\frac{k-2\alpha -1}{e} \right)^{k-2\alpha -1}(1+o(1)) . $$ 
%Furthermore
%$$\Gamma(k-2\alpha)^{-1} \int_{0}^{t_1} t^{k-2\alpha-1}e^{-t}dt =o(1) $$
%and therefore $D_k$ is scale-free distributed with exponent $(-1-2\alpha)$ 
%\begin{equation}
%\label{eq:sequence_large_degree}
%\mathbb{E}[D_k]=n\cdot (1+o(1)) 2\alpha e^{-\alpha C} \left(\frac{2\alpha}{\pi (\alpha -1/2)} \right)^{2\alpha}\cdot k^{-1-2\alpha}. 
%\end{equation}

The last ingredient in the proof of Theorem~\ref{thm:degree_seq} is to show that $D_k$ is concentrated around its expectation. To this end, we will use the following large deviation inequality. Let $f$ be a function on the random variables $X_1, \dots, X_n$ that take values in some set $A_i$. We say that $f$ is Lipschitz with coefficients $c_1\dots c_n$ and bad event $\mathcal{B}$ if for all $x,y\in A$ 
$$\left|\mathbb{E}[f|X_{1},\dots X_{i-1}, X_i=x, \overline{\mathcal{B}}]-\mathbb{E}[f|X_{1},\dots X_{i-1}, X_i=y, \overline{\mathcal{B}}]\right|\le c_i .$$
(We denote by $\overline{\mathcal{B}}$ the complement of $\mathcal{B}$.)
Then the following estimates are true.
\begin{theorem}[Theorem~7.1 in \cite{dubhashi2009concentration}]
\label{lem:concentration}
Let $f$ be a function of $n$ independent random variables $X_1,\dots, X_n$, each $X_i$ taking values in a set $A_i$, such that $\mathbb{E}[f]$ is bounded. Assume that 
$$m\le f(X_1, \dots, X_n)\le M.$$
Let $\mathcal{B}$ any event, and let $c_i$ be the maximum effect of $f$ assuming the complement $\overline{\mathcal{B}}$ of $\mathcal{B}$:
$$\max_{x,y}|\mathbb{E}[f|X_1,\dots, X_{i-1}, X_i=x, \overline{\mathcal{B}}]-\mathbb{E}[f|X_1,\dots, X_{i-1}, X_i=y, \overline{\mathcal{B}}] | \le c_i.$$
 Then
$$\Pr[f> \mathbb{E}[f]+t+(M-m)\Pr[\mathcal{B}]] \le e^{-{2t^2}/{\sum_i c_i^2}} +\Pr[\mathcal{B}]$$
and
$$\Pr[f< \mathbb{E}[f]-t-(M-m)\Pr[\mathcal{B}]] \le e^{-{t^2}/{\sum_i c_i^2}} +\Pr[\mathcal{B}].$$
\end{theorem}
In our setting, $D_k$ is obviously a function of $X_1, \dots , X_n$, where $X_i$ denotes the coordinates of the $i$th vertex. Then the following lemma says that the above theorem is applicable in our setting.
\begin{lemma}
\label{lem:lipschitz}
Let $\alpha > 1/2$ and $0<\beta<1$. There is a constant~$c>0$ such that~$D_k(\beta)$ is Lipschitz with~$c_i\le cn^{1-\beta}+1$ and bad event $\mathcal{B}$, where
$$\mathcal{B}:=\left\{\text{there is a vertex in~$O(\beta) = B_0(R)\setminus B_0(\beta R)$ with degree at least~$cn^{1-\beta}$}\right\}.$$
Moreover, $\Pr[\mathcal{B}]=e^{-n^{\Omega(1-\beta)}}.$
\end{lemma}
\begin{proof}
Note that unless~$\mathcal{B}$ holds every vertex in~$O:=O(\beta)$ is connected to at most~$cn^{1-\beta}$ other vertices in~$O$. Therefore, any change in~$X_i$ can increase or decrease the number of vertices in~$O$ of degree~$k$ by at most~$cn^{1-\beta}+1$ (the additional ``+1'' is due to the fact that vertex $i$ could change its degree as well). It remains to bound the probability of~$\mathcal{B}$.
By applying Lemma~\ref{lem:monotone} we see that the expected degree in $O$ of a vertex with radius $r\geq \beta R$ is at most
$$n\cdot \mu(B_0(R)\cap B_{\beta R}(R)\setminus B_0(\beta R))\stackrel{\textrm{(Lem.\ \ref{lem:intersection_area})}}{=}O\left(n\cdot e^{-\frac{\beta R}{2}} \right) =O(n^{1-\beta}) .$$
Hence the expected degree of a vertex of radius at least $\beta R$ is at most $c'n^{1-\beta}$ for some constant $c'$. For $c:=2ec'$ it suffices to apply a Chernoff bound to show that for a vertex $v$ of radius at least $\beta R$
$$\Pr[d_O(v)>cn^{1-\beta}] \le 2^{-cn^{1-\beta}} .$$
The statement of the lemma follows by union bound over all vertices. 
\end{proof}
\begin{proof}[Proof of the first part of Theorem~\ref{thm:degree_seq}]
Set $\beta:= \max\{\frac{3}{5}, 1/(2\alpha), 1-\frac{1}{4\alpha}\}+\varepsilon$, where $\varepsilon > 0$ will be chosen later such that $\beta <1$. The total number of vertices of degree $k$, for any $k$ in the considered range, is at most 
\begin{equation}
\label{eq:degkupper}
D_k(\beta)+|I(\beta)|+e(I(\beta),O(\beta))
\end{equation}
and at least 
\begin{equation}
\label{eq:degklower}
D_k(\beta)-e(I(\beta),O(\beta)) ,
\end{equation}
since every vertex in $I$ could possible have degree $k$, and since each edge counted in $e(I,O)$ may affect the degree of one vertex in $O$. We will argue in the sequel that the contribution of $|I|$ and $e(I,O)$ is with high probability negligible in the above equations. 

First, since $\beta \ge 1 - \frac1{4\alpha}$, by applying Lemma~\ref{lem:few_vertices_I} we obtain that with probability at least $1 - e^{-n^{\Omega(1)}}$,
\begin{equation}
\label{eq:Iupper}
|I(\beta)|=O\left(n^{1-2\alpha(1-\beta)}\right).
\end{equation}
Moreover, Lemma~\ref{lem:few_edges_IO} yields that with high probability
\begin{equation}
\label{eq:eIOupper}
e(I(\beta),O(\beta))=O\left(n^{1-(2\alpha-1)(1-\beta)}\log n\right) .
\end{equation}
It remains to determine the value of $D_k$. Our assumptions on $k$ guarantee that $k\le n^{\delta'}$, where $\delta' < \frac{(2\alpha-1)(1-\beta)}{2\alpha+1}$, provided that $\varepsilon>0$ is sufficiently small. Additionally, we claim that $\delta' < 2(2\beta -1)$. To see this, note that since $a > 1/2$
\[
\frac{(2\alpha-1)(1-\beta)}{2\alpha+1} < 2(2\beta-1) \Leftrightarrow \beta > \frac{6\alpha + 1}{10 \alpha + 3} =: h(\alpha).
\]
But $h(\alpha)$ is increasing, and thus it is maximized at $\alpha = \infty$, where $\lim_{\alpha \to \infty}h(\alpha) = 3/5$. This shows that indeed $\delta' < 2(2\beta -1)$. With all these facts at hand we can apply Lemma~\ref{lem:degree_sequence}, which implies that
\begin{equation}
\label{eq:d_k_ass}
\mathbb{E}[D_k(\beta)]= \Theta(nk^{-(2\alpha+1)}) = \Omega(n^{1- (2\alpha+1)\delta'}) \stackrel{(\delta' < \frac{(2\alpha-1)(1-\beta)}{2\alpha+1})}{=} \omega\left(n^{1-(2\alpha-1)(1-\beta)}\log n\right).
\end{equation}
We apply Theorem~\ref{lem:concentration} with $f:=D_k(\beta)$, $t:=n^{3/2-\beta+2\alpha\varepsilon}$ and Lipschitz coefficients $c_i$ and 'bad' event $\mathcal{B}$ as stated in Lemma~\ref{lem:lipschitz}. Note that $M=n$ and therefore $M\cdot \Pr[\mathcal{B}]=o(1)$. It follows that
\[
	\Pr[|D_k(\beta) - \Exp[D_k(\beta)]| \ge t + o(1)] \le 2e^{-\Omega(t^2/n^{1 + 2(1-\beta)})} + e^{-n^{\Omega(1)}}
	= e^{-n^{\Omega(1)}}.
\]
However, $\beta \ge 1 - \frac1{4\alpha} + \varepsilon$ implies for all $0 \le k \le n^{\delta'}$ that
\[
	\Exp[D_k(\beta)] = \omega \left(n^{1-(2\alpha-1)(1-\beta)}\right) = \omega\left(n^{3/2-\beta+2\alpha\varepsilon}\right) = \omega(t).
\]
This shows that with probability at least $1 - e^{-n^{\Omega(1)}}$ we have for every $k$ in the considered range that $D_k(\beta) = (1 + o(1))\Exp[{D_k(\beta)}]$. Together with~\eqref{eq:degkupper}--\eqref{eq:d_k_ass} the proof of the theorem is completed.
\end{proof}

